Requirements Quality Research Artifacts: Recovery, Analysis, and Management Guideline

Requirements quality research, which is dedicated to assessing and improving the quality of requirements specifications, is dependent on research artifacts like data sets (containing information about quality defects) and implementations (automatically detecting and removing these defects). However, recent research exposed that the majority of these research artifacts have become unavailable or have never been disclosed, which inhibits progress in the research domain. In this work, we aim to improve the availability of research artifacts in requirements quality research. To this end, we (1) extend an artifact recovery initiative, (2) empirically evaluate the reasons for artifact unavailability using Bayesian data analysis, and (3) compile a concise guideline for open science artifact disclosure. Our results include 10 recovered data sets and 7 recovered implementations, empirical support for artifact availability improving over time and the positive effect of public hosting services, and a pragmatic artifact management guideline open for community comments. With this work, we hope to encourage and support adherence to open science principles and improve the availability of research artifacts for the requirements research quality community.

==> variables.tex <==
\newcommand\nauthors{40} % number of authors approached during the J3RE initiative
\newcommand\nauthorsnew{5} % number of new authors approached (in contrast to 3RE)
\newcommand\requestcompleted{21} % number of author request currently in status code Completed
\newcommand\requestcompletedperc{52.5} % percentage of author requests currently in status code Completed
\newcommand\requestanswered{30} % number of author request currently in status code Answered
\newcommand\requestansweredperc{75.0} % percentage of author requests currently in status code Answered
\newcommand\requestunanswered{8} % number of author request currently in status code Unanswered
\newcommand\requestunansweredperc{20.0} % percentage of author requests currently in status code Unanswered
\newcommand\requestundeliverable{2} % number of author request currently in status code Undeliverable
\newcommand\requestundeliverableperc{5.0} % percentage of author requests currently in status code Undeliverable
\newcommand\daysresponse{23.8} % average number of days until the first response to a request
\newcommand\dayscomplete{29.25} % average number of days until the request was completed
\newcommand\datasetsimproved{10} % number of datasets with improved availability
\newcommand\datasetsimprovedperc{17.5} % percentage of datasets with improved availability
\newcommand\datasetsclarified{30} % number of datasets with same (or worse) but clarified availability
\newcommand\datasetsclarifiedperc{52.6} % percentage of datasets with same (or worse) but clarified availability
\newcommand\datasetsaddressed{40} % number of datasets addressed during the scope of the initiative
\newcommand\datasetsaddressedperc{70.1} % percentage of datasets addressed during the scope of the initiative
\newcommand\datasetsarchived{8} % number of datasets disclosed according to open science principles
\newcommand\datasetsarchivedperc{14.0} % percentage of datasets disclosed according to open science principles
\newcommand\datasetsavailable{15} % number of datasets currently available
\newcommand\datasetsavailableperc{26.3} % percentage of datasets currently available
\newcommand\datasetslost{19} % number of {t}s excused as {excuse}
\newcommand\datasetssensitive{11} % number of {t}s excused as {excuse}
\newcommand\implementationsimproved{7} % number of implementations with improved availability
\newcommand\implementationsimprovedperc{19.4} % percentage of implementations with improved availability
\newcommand\implementationsclarified{10} % number of implementations with same (or worse) but clarified availability
\newcommand\implementationsclarifiedperc{27.7} % percentage of implementations with same (or worse) but clarified availability
\newcommand\implementationsaddressed{17} % number of implementations addressed during the scope of the initiative
\newcommand\implementationsaddressedperc{47.2} % percentage of implementations addressed during the scope of the initiative
\newcommand\implementationsarchived{6} % number of implementations disclosed according to open science principles
\newcommand\implementationsarchivedperc{16.6} % percentage of implementations disclosed according to open science principles
\newcommand\implementationsavailable{11} % number of implementations currently available
\newcommand\implementationsavailableperc{30.5} % percentage of implementations currently available
\newcommand\implementationslost{6} % number of {t}s excused as {excuse}
\newcommand\implementationsproprietary{4} % number of {t}s excused as {excuse}
